MV-Map: Offboard HD-Map Generation with Multi-view Consistency

While bird's-eye-view (BEV) perception models can be useful for building high-definition maps (HD-Maps) with less human labor, their results are often unreliable and demonstrate noticeable inconsistencies in the predicted HD-Maps from different viewpoints. This is because BEV perception is typically set up in an 'onboard' manner, which restricts the computation and consequently prevents algorithms from reasoning multiple views simultaneously. This paper overcomes these limitations and advocates a more practical 'offboard' HD-Map generation setup that removes the computation constraints, based on the fact that HD-Maps are commonly reusable infrastructures built offline in data centers. To this end, we propose a novel offboard pipeline called MV-Map that capitalizes multi-view consistency and can handle an arbitrary number of frames with the key design of a 'region-centric' framework. In MV-Map, the target HD-Maps are created by aggregating all the frames of onboard predictions, weighted by the confidence scores assigned by an 'uncertainty network'. To further enhance multi-view consistency, we augment the uncertainty network with the global 3D structure optimized by a voxelized neural radiance field (Voxel-NeRF). Extensive experiments on nuScenes show that our MV-Map significantly improves the quality of HD-Maps, further highlighting the importance of offboard methods for HD-Map generation.

==> figtex/semi_supervised.tex <==
\begin{table}[t]
    \centering
    \caption{We compare the onboard model trained on the ground truth label with one using the pseudo label generated by our offboard fusion network. We use 50 scenes to train our online baseline model and evaluate on the remaining 100 scenes in the validation set.}
    \label{tb:semi-supervised}
    \vspace{-2mm}
    \resizebox{0.95\linewidth}{!}{
    \begin{tabular}{l|cccc}
    \toprule
    \multirow{2}{*}{Label Type} & \multicolumn{4}{c}{mIoU} \\ & Divider & Ped Crossing & Boundary & All   \\ 
    \midrule
    Baseline       & --  & -- & -- & -- \\
    \midrule
    GT Label   & --  & --  & -- & -- \\
    Pseudo Label   & --  & --  & -- & -- \\
    \bottomrule
    \end{tabular}
    }
    \vspace{-4mm}
\end{table}

==> sections/supp_main.tex <==
This supplementary material contains the following contents:
\begin{enumerate}[leftmargin=*, noitemsep, nolistsep, label=(\Alph*)]
    \item \textbf{Demo video.} We provide a demo for offboard HD-Map generation in Sec.~\ref{supsec:video_demo}.
    \item \textbf{Voxel-NeRF details.} We explain the formulation of training and using Voxel-NeRFs in Sec.~\ref{supsec:voxel_nerf}.
    \item \textbf{Generalizability of \ourmodel with LiDAR.} In addition to the vision-oriented experimentation in the main paper, we show the generalizability of \ourmodel and incorporate it with the LiDAR modality in Sec.~\ref{supsec:lidar}.%formulation and 
    \item \textbf{Applications of Auto-labeling.} We validate the effectiveness of \ourmodel for auto-labeling, by using it to generate pseudo HD-Map labels in Sec.~\ref{supsec:auto_labeling}.%training BEV perception models
    \item \textbf{Additional quantitative results.} We supplement ablation studies, especially using additional onboard models, in Sec.~\ref{supsec:quantitative}.
    \item \textbf{Additional qualitative results.} The generated HD-Maps together with the reconstructed 3D structure via our Voxel-NeRF are visualized in Sec.~\ref{sec:vis-nerf}.
    \item \textbf{Implementation details.} We describe additional implementation details for reproducing our results in Sec.~\ref{supsec:implementation}. We will also publicly release our code and trained models upon acceptance.
\end{enumerate}

\section{Demo Video}
\label{supsec:video_demo}

We provide a demo video in the supplementary material that showcases how our \ourmodel produces high-quality HD-Maps by fusing frames from diverse viewpoints. Notably, the video highlights the effectiveness of \ourmodel in {\em iteratively refining} complex road topologies and long road elements while dealing with frequent occlusions in urban traffic.
% We provide a demo video in the supplementary material that showcases how our \ourmodel fuses high-quality HD-Maps with frames from diverse viewpoints. The video highlights the {\em iterative refinement} of complex road topologies and long road elements under frequent occlusions in urban traffic.

\input{supp_sections/experiments}
\input{supp_sections/extra}
\input{supp_sections/implementations}

==> supp_sections/tables/hdmapnet.tex <==
\begin{table}[tb]
\caption{MV-Map generalizes to other onboard models. Using HDMapNet~\cite{li2022hdmapnet} with both camera and LiDAR modalities as our onboard model, \ourmodel is consistently effective and significantly improves the HD-Map quality. We evaluate under the same short-range setting as HDMapNet.} \vspace{-2mm}
    \centering
    \resizebox{0.99\linewidth}{!}{
    \begin{tabular}{c|cccc}
    \toprule
    \multirow{2}{*}{\ourmodel} & 
    \multicolumn{4}{c}{mIoU (Short-range)} \\ & Divider & Ped Crossing & Boundary & All   \\ 
    \midrule
    \xmark & 46.20  & 24.38  & 56.99 & 42.52 \\
    \cmark & \textbf{49.82}  & \textbf{29.83}  & \textbf{58.54} & \textbf{46.06} \\
    \bottomrule
    \end{tabular}
    }
    
    \vspace{-2mm}
    \label{tb:supp-encoder-hdmapnet}
\end{table}

==> tables/fusion_frames.tex <==
\begin{table}[t]
    \centering
    \resizebox{0.95\linewidth}{!}{
    \begin{tabular}{l|cccc}
    \toprule
    \multirow{2}{*}{\#Frames} & \multicolumn{4}{c}{mIoU} \\ & Divider & Ped Crossing & Boundary & All   \\ 
    \midrule
    1 (online) & 39.30  & 26.44  & 39.10  & 34.95 \\
    \midrule
    3        & 40.93  & 27.65  & 41.19 & 36.59 \\
    5        & 41.96  & 28.43  & 42.46 & 37.62 \\
    7        & 42.83  & 29.17  & 43.52 & 38.51 \\
    15       & 45.38  & 31.88  & 46.74 & 41.33 \\
    All (global) & \textbf{48.15} & \textbf{33.34}  & \textbf{50.28} & \textbf{43.92} \\
    \bottomrule
    \end{tabular}
    }
    \caption{Ablation on different numbers of fusion frames in long-range settings (100m $\times$ 100m). Our uncertainty-aware fusion benefits from more frames of information.}
    \label{tb:fusion-frames}

\end{table}
